CARE: Causality Reasoning for Empathetic Responses by Conditional Graph Generation

Recent approaches to empathetic response generation incorporate emotion causalities to enhance comprehension of both the user's feelings and experiences. However, these approaches suffer from two critical issues. First, they only consider causalities between the user's emotion and the user's experiences, and ignore those between the user's experiences. Second, they neglect interdependence among causalities and reason them independently. To solve the above problems, we expect to reason all plausible causalities interdependently and simultaneously, given the user's emotion, dialogue history, and future dialogue content. Then, we infuse these causalities into response generation for empathetic responses. Specifically, we design a new model, i.e., the Conditional Variational Graph Auto-Encoder (CVGAE), for the causality reasoning, and adopt a multi-source attention mechanism in the decoder for the causality infusion. We name the whole framework as CARE, abbreviated for CAusality Reasoning for Empathetic conversation. Experimental results indicate that our method achieves state-of-the-art performance.

==> OutLet.tex <==
\section{Introduction}
Empathy is the capability to perceive and understand affective states and acting of another individual accordingly \cite{paiva2017empathy,decety2004functional}. As a broad and complex construct, empathy is composed of both an affective and a cognitive component \cite{davis1983measuring}. The affection correlates to understanding of the other's emotion and corresponding emotional reactions \cite{hoffman2001empathy}, while cognition corresponds to comprehension and reasoning of the other's situation and experiences \cite{preston2002empathy}.
% Both aspects, especially the cognition, require the capability of reasoning and inference  \cite{wondra2015appraisal}.

Earlier work on empathetic response generation merely consider the affection through investigation of the user's emotion and the response emotion \cite{moel,majumder2020mime,li2019empgan}, which limits empathetic expression. 
Therefore, recent work has started to take the affection and the cognition into account meanwhile by incorporation of emotion causes and effects \cite{wang2021empathetic,gao-etal-2021-improving-empathetic,Kim:2021:empathy,CEM2021}. 
Despite notable improvements, these approaches suffer from two critical problems. 
The first problem is that they merely consider to detect causes and effects of the user's emotion state, which are merely parts of cognition. Some other causal reasoning, which is not related to emotion states directly, is also necessary for understanding of the user's situation and experiences. 
Another problem is that their methods detect emotion causes and effects independently and ignore global intra-causality structures.
Due to above two problems, their understanding of the user's situation and experiences is insufficient. 
% As a result, they tend to generate relevant but unreasonable responses, as if they pretend to be interested in what the user is talking and respond based on some random fragment in the user's utterances. 
% i.e., causal relationships between (\romannumeral1) emotion and causality, and (\romannumeral2) causality and causality.

\begin{figure}
    \centering
    \includegraphics{Figure/fig-overview.pdf}
    \caption{The overview of our proposed framework. The solid lines represent modules or data used for both posterior and prior computation, while the dot lines represent modules or data used only for posterior computation.}
    \label{fig:CVGAE}
\end{figure}

% 这个地方想下怎么体积matrix，方便别人理解。
% To capture and leverage intra-causality structures, we propose to reason all plausible causal relationships .
To solve above problems, we propose to reason all plausible causal relationships simultaneously with the user's emotion as the condition.
Inspired by variational graph auto-encoders \cite{kipf2016variational}, which uses latent variables for graph generation, we design a conditional variational graph auto-encoder (CVGAE) to reason relationships among nodes in a graph given certain condition. The connection between our CGAVE and GVAE is like that between CVAE \cite{sohn2015learning} and VAE \cite{kingma2013auto}.
We use CVGAE to infer whether there is a causal relationship between any two nodes. Each node\footnote{The part of speech of the node can be verb, noun, adjective, or adverb} is a word that can represent the user's states or actions. The condition is a combination of dialogue context, the user's emotion, and plausible future dialogue content.
By doing so, we not only construct the intra-causality structures, but also identify emotion causes and effects that are suitable for the conversation.

In this paper, we propose a novel model named GREmp (\textbf{G}raph-based \textbf{R}easoning for \textbf{Emp}athetic response generation). 
Based on transformer-based response generation model, GREmp predicts emotional causal relations by a CVGAE model to provide emotional causal information for decoding. To train the CVGAE, we use user's utterances in the future conversation and a causal knowledge graph as the supervision signal.
The decoder absorbs the emotional causal information by a multi-source attention mechanism. 
We train the model in an end-to-end manner.
Experimental results demonstrate that our method is capable of reasoning the emotion-related causal relationships, and generating more empathetic responses than the previous state-of-the-art method. 

Our main contributions are three-fold:
\begin{enumerate}[leftmargin=*,label=\arabic*).]
    \item We introduce CVGAE for structured prediction and relationship reasoning under conditions, and use it to reason emotional causal relations.
    \item We propose to consider intra-causality structures for a deeper understanding of emotion causes and effects for improvement of empathetic expression.
    \item We design a model named GREmp, which leverages emotion causes and effects for empathetic response generation, and test it on a benchmark \textsc{EmpatheticDialogues}.
\end{enumerate}
% Experimental results suggest that GREmp is able to predict emotion-related causal relationships, and generate more empathetic and informative responses compared with the previous methods.

As shown in \Cref{fig:CVGAE}, model A, representing previous models, identifies \textit{bowling-ball game} as the reason of \textit{impressive} emotion due to its more space (two words) in detected emotion causes. However, \textit{brother}, which involves more to causal relations, should be the main focus to understand the user.


Empathy is the capability to perceive and understand affective states and acting of another individual, and respond accordingly \cite{paiva2017empathy,decety2004functional}. It is composed of both affection and cognition \cite{davis1983measuring}. The affection correlates to understanding of the other's emotion and corresponding emotional reactions \cite{hoffman2001empathy}, while cognition corresponds to comprehension and reasoning of the other's situation and experiences \cite{preston2002empathy}.


Recent approaches to empathetic response generation incorporate emotion causalities for comprehension of both the user's feelings and experiences.
However, they suffer from two critical issues. 
The first is that they merely consider direct causes and effects of the user's emotion, and ignore causal relationships among experiences. 
The second issue is that they neglect interdependence among causalities, and detect causal relationships independently.
To solve above problems, we design conditional variational graph auto-encoders (CVGAE) to reason all plausible causal relationships interdependently given the user's emotion and conversation context. For empathetic responses, we propose a model named CARE
(\textbf{C}onditional c\textbf{A}usality \textbf{R}easoning for \textbf{E}mpathetic chatbot), which takes both causalities reasoned by CVGAE and conversation context as inputs to generate final responses. Experimental results indicate that our method can achieve state-of-the-art performances and generate more empathetic responses than previous models. 


In specific, we detect whether there is a causal relationship between any two nodes in Causes Effect Graph (CEG)\footnote{Each node in CEG is one of verb, noun, adjective, and adverb, and is able to describe the user's state or action} \cite{ijcai2020-guided}, a causal knowledge graph. The reasoning is under a certain condition, which combines the user's emotion, dialogue context, and predicted future dialogue content, to fit the user's feelings and experiences. 
